Model-Based Reinforcement Learning Exploiting State-Action Equivalence

Leveraging an equivalence property in the state-space of a Markov Decision Process (MDP) has been investigated in several studies. This paper studies equivalence structure in the reinforcement learning (RL) setup, where transition distributions are no longer assumed to be known. We present a notion of similarity between transition probabilities of various state-action pairs of an MDP, which naturally defines an equivalence structure in the state-action space. We present equivalence-aware confidence sets for the case where the learner knows the underlying structure in advance. These sets are provably smaller than their corresponding equivalence-oblivious counterparts. In the more challenging case of an unknown equivalence structure, we present an algorithm called ApproxEquivalence that seeks to find an (approximate) equivalence structure, and define confidence sets using the approximate equivalence. To illustrate the efficacy of the presented confidence sets, we present C-UCRL, as a natural modification of UCRL2 for RL in undiscounted MDPs. In the case of a known equivalence structure, we show that C-UCRL improves over UCRL2 in terms of regret by a factor of $\sqrt{SA/C}$, in any communicating MDP with $S$ states, $A$ actions, and $C$ classes, which corresponds to a massive improvement when $C \ll SA$. To the best of our knowledge, this is the first work providing regret bounds for RL when an equivalence structure in the MDP is efficiently exploited. In the case of an unknown equivalence structure, we show through numerical experiments that C-UCRL combined with ApproxEquivalence outperforms UCRL2 in ergodic MDPs.

==> New folder/C-UCRL_regret.tex <==

In this section, we prove Theorem \ref{thm:regretKnownC}, which provides an upper bound on the regret of \CUCRL$(\cC,\boldsymbol\sigma)$. We provide the proof for the case when the reward function is unknown to the learner too.
Our proof follows similar lines as in the proof of \cite[Theorem~2]{jaksch2010near}.
We first provide the following time-uniform concentration inequality to control a bounded martingale difference sequence, which follows from time-uniform Laplace concentration inequality:


%\begin{lemma}[Uniform confidence intervals]\label{lem:confintervals}
%	Let $Y_1,\dots Y_t$ be a sequence of $t$ i.i.d.~real-valued random variables with mean $\mu$, such that $Y_t-\mu$ is $\sigma$-sub-Gaussian. Let
%	$\mu_t= \frac{1}{t}\sum_{s=1}^t Y_s$ be the empirical mean estimate. Then, for all $\delta\in(0,1)$, it holds
%	\beqan
%	\Pr\bigg(\exists t\in\Nat,\quad |\mu_t -\mu| \geq \sigma\sqrt{\Big(1+\frac{1}{t}\Big)\frac{2\ln\big(\sqrt{t+1}/\delta\big)}{t}}\bigg)& \leq& \delta\,.
%	\eeqan		
%\end{lemma}

\begin{lemma}[Time-uniform Azuma-Hoeffding]\label{lem:time-uniform-AzumaHoeffding}
	Let $(X_t)_{t\geq 1}$ be a martingale difference sequence bounded by $b$ for some $b>0$  (that is, $|X_t|\leq b$ for all $t$). Then, for all $\delta\in (0,1)$,
	\beqan
	\mathbb P\bigg(\exists T \in\Nat: \sum_{t=1}^T  X_t \geq b\sqrt{ 2(T+1) \log\big( \sqrt{T+1}/\delta\big)}\bigg) \leq \delta\,.
	\eeqan
\end{lemma}



\begin{proof}\textbf{(of Theorem \ref{thm:regretKnownC})} Let $\delta\in (0,1)$. To simplify notations, we define the short-hand $J_k:=J_{t_k}$ for various random variables that are fixed within a given episode $k$ (for example $\cM_{k}:=\cM_{t_k}$). Denote by $m(T)$ the number of episodes initiated by the algorithm up to time $T$.
An application of Lemma \ref{lem:time-uniform-AzumaHoeffding} yields:
\als{
\kR(T)&= \sum_{t=1}^T g_\star- \sum_{t=1}^T r_t(s_t,a_t) \leq \sum_{s,a} N_{m(T)}(s,a)(g_\star - \mu(s,a)) + \sqrt{ \tfrac{1}{2}(T+1) \log( \sqrt{T+1}/\delta)}\, ,
}
with probability at least $1-\delta$. We have
\als{
\sum_{s,a} N_{m(T)}(s,a)(g_\star - \mu(s,a)) &= \sum_{k=1}^{m(T)}  \sum_{s,a}  \sum_{t=t_k+1}^{t_{k+1}}\indic{s_t=s,a_t=a} \big(g_\star - \mu(s,a)\big)\\
&= \sum_{k=1}^{m(T)}  \sum_{s,a}  \nu_k(s,a)\big(g_\star - \mu(s,a)\big)\,.
}
Defining $\nu_k(c):=\sum_{s,a} \nu_k(s,a)$ for $c\in \cC$, we further obtain
\als{
\sum_{s,a} N_{m(T)}(s,a)(g_\star - \mu(s,a)) &= \sum_{k=1}^{m(T)}  \sum_{c\in\cC}  \nu_k(c) \big(g_\star - \mu(c)\big) \, ,
}
where we have used that $\mu(s,a)$ has constant value $\mu(c)$ for all $(s,a)\in c$. For $1\leq k\leq m(T)$, we define the regret of episode $k$ as
$\Delta_k = \sum_{c\in\cC}\nu_k(c) \big(g_\star - \mu(c)\big)$. Hence, with probability at least $1-\delta$,
\als{
\kR(T) \leq \sum_{k=1}^{m(T)} \Delta_k + \sqrt{ \tfrac{1}{2}(T+1) \log( \sqrt{T+1}/\delta)}\, .
}
We say an episode is \emph{good} if $M \in \cM_{k}$ (that is, the set $\cM_{k}$ of plausible MDPs contains the true model), and \emph{bad} otherwise.

\paragraph{Control of the regret due to bad episodes ($M \notin \cM_{k}$).}
Due to using time-uniform instead of time-instantaneous confidence bounds, we can show that with high probability, all episodes are good for $T\in \Nat$. More precisely,
with probability higher than $1-2\delta$, for all $T$, bad episodes do not contribute to the regret:
\beqan
\sum_{k=1}^{m(T)}\Delta_k\indic{M \notin \cM_{k}} = 0\,.
\eeqan

\paragraph{Control of the regret due to good episodes ($M \in \cM_{k}$).} We closely follow \citep{jaksch2010near} and decompose the regret to control the transition and reward functions.
At a high level, we make two major modifications as follows. (i) We use the time-uniform bound stated in Lemma \ref{lem:time-uniform-AzumaHoeffding} to control the martingale difference sequence that appears; and
(ii) as the stopping criterion of \CUCRL($\cC,\boldsymbol\sigma$) slightly differs from that of \UCRL, we use the following lemma to control the number $m(T)$ of episodes:
\begin{lemma}[Number of episodes]\label{lem:NbEpisodes}
	The number $m(T)$ of episodes of \CUCRL($\cC,\boldsymbol\sigma$) up to time $T \geq C$ is upper bounded by:
	\begin{equation*}
	m(T) \leq C\log_2(\tfrac{8T}{C})\, .
	\end{equation*}
\end{lemma}


Consider a good episode $k$ (hence, $M \in \cM_{k}$). The \texttt{EVI} algorithm outputs a policy $\pi^+_{k}$ and $\widetilde M_{k}$ satisfying  $g_{\pi^+_{k}}^{\widetilde M_{k}} \geq g_\star - \frac{1}{\sqrt{t_k}}$. Let us define $g_k:= g_{\pi^+_{k}}^{\widetilde M_{k}}$. It then follows that
\begin{equation}
\Delta_k = \sum_{c \in \cC} \nu_k(c) \big(g_\star - \mu(c)\big) \leq \sum_{c \in \cC} \nu_k(c)
\big(g_k - \mu(c)\big) + \sum_{c \in \cC} \frac{\nu_k(c)}{\sqrt{t_k}} \, .
\label{eq:delta_init}
\end{equation}
Using the same argument as in the proof of \cite[Theorem~2]{jaksch2010near}, the value function $u_k^{(i)}$ computed by \texttt{EVI} at the last iteration $i$ satisfies: $\max_{s} u_k^{(i)}(s) - \min_{s} u_k^{(i)}(s) \!\leq\! D$. Moreover, the convergence criterion of \texttt{EVI} implies
\begin{equation}
|u_k^{(i+1)}(s) - u_k^{(i)}(s) - g_k| \leq \frac{1}{\sqrt{t_k}}\,, \qquad  \forall s \in \cS\, .
\label{eq:puterman_convergence}
\end{equation}

By the design of \texttt{EVI}, we have
$
u_k^{(i+1)}(s) = \widetilde\mu_{k}(s,\pi^+_{k}(s)) + \sum_{x} \widetilde p_k(x|s,\pi^+_{k}(s)) u_k^{(i)}(x) \,.
$
Substituting this into (\ref{eq:puterman_convergence}) gives
\begin{equation*}
\Big|\Big( g_k - \widetilde\mu_{k}(s,\pi_k^+(s)) \Big) - \Big(\sum_{x} \widetilde p_{k}(x|s,\pi_k^+(s))u_k^{(i)}(x) - u_k^{(i)}(s)\Big)\Big|
\leq \frac{1}{\sqrt{t_k}}\, , \qquad \forall s\in \cS\, .
\end{equation*}
Defining
${\bf g}_k = g_k \mathbf 1$, $\widetilde{\boldsymbol{\mu}}_{k} := \big(\widetilde\mu_{k}(s,\pi_k^+(s))\big)_{s\in \cS}$, $\widetilde{\mathbf{P}}_k := \big(\widetilde p_{k}(x|s,\pi_k^+(s))\big)_{s, x\in \cS}$, and $\nu_{k} := \big(\nu_k\big(s,\pi_k^+(s))_{s\in \cS}$, we can rewrite the above inequality as:
\begin{equation*}
\Big|{\bf g}_k - \widetilde{\boldsymbol{\mu}}_{k} - (\widetilde{\mathbf{P}}_k - \mathbf{I}) u_k^{(i)} \Big|
\leq \frac{1}{\sqrt{t_k}}\mathbf 1\,.
\end{equation*}
Combining this with (\ref{eq:delta_init}) yields
\begin{align}
\Delta_k&\leq \sum_{s,a} \nu_k(s,a) \big(g_k-\mu(s,a)\big) + \sum_{s,a} \frac{\nu_k(s,a)}{\sqrt{t_k}} \nonumber\\
&= \sum_{s,a} \nu_k(s,a) \big( g_k - \widetilde\mu_{k}(s,a) \big) + \sum_{s,a} \nu_k(s,a) \big( \widetilde\mu_{k}(s,a) - \mu(s,a) \big) + \sum_{s,a}
\frac{\nu_k(s,a)}{\sqrt{t_k}} \nonumber\\
&\leq \nu_{k} (\widetilde{\mathbf{P}}_k - \mathbf{I} ) u_k^{(i)} + \sum_{s,a} \nu_k(s,a) \big(\widetilde\mu_{k}(s,a) - \mu(s,a) \big) + 2 \sum_{s,a} \frac{\nu_k(s,a)}{\sqrt{t_k}}\, .\nonumber
\end{align}
Similarly to \citep{jaksch2010near}, we define $w_k(s) := u_k^{(i)}(s) - \tfrac{1}{2}(\min_s u_k^{(i)}(s) + \max_s u_k^{(i)}(s))$ for all $s\in \cS$. Then, in view of the fact that $\widetilde{\mathbf{P}}_k$ is row-stochastic, we obtain



\begin{align}
\Delta_k&\leq \nu_{k} (\widetilde{\mathbf{P}}_k - \mathbf{I} ) w_k + \sum_{s,a} \nu_k(s,a) \big(\widetilde \mu_{k}(s,a) - \mu(s,a) \big) + 2 \sum_{s,a} \frac{\nu_k(s,a)}{\sqrt{t_k}}\, .
\end{align}
The second term in the right-hand side can be upper bounded as follows. Fix pair $(s,a)$ and let $c_{s,a}$ denote the cluster to which $(s,a)$ belongs. The fact $M \in \cM_{k}$ implies
\als{
\widetilde\mu_{k}(s,a) - \mu(s,a) &\leq |\widetilde\mu_{k}(s,a) - \widehat \mu_{k}(s,a)| + |\widehat \mu_{k}(s,a) - \mu(s,a)| \leq 2\beta'_{n_{k}(c_{s,a})}(\tfrac{\delta}{C}) \\
    &= 2\sqrt{\frac{1}{2n_{k}(c_{s,a})}\Big(1\!+\!\frac{1}{n_{k}(c_{s,a})}\Big)\log\Big(C\sqrt{n_{k}(c_{s,a})\!+\!1}/\delta\Big)} \\
    &\leq 2\sqrt{\frac{1}{n_k(c_{s,a})}\log\big(C\sqrt{T+1}/\delta\big)}\, ,
}
where we have used $1\leq n_k(c_{s,a}) \leq T$ in the last inequality. Using this bound and noting that $t_k\geq n_k(c)$, we obtain
\begin{align}
\Delta_k
&\leq \nu_{k} (\widetilde{\mathbf{P}}_k-\mathbf{I})w_k + 2\Big(\sqrt{\log\big(C\sqrt{T+1}/\delta\big)} + 1\Big)
\sum_{c\in \cC} \frac{\nu_k(c)}{\sqrt{n_{k}(c)}}\, .
\label{eq:main_delta_minmk}
\end{align}



\begin{comment}

{\color{blue}Using the Bellman operator on the optimistic MDP:
\als{
u_k^{(i+1)}(s) = \widetilde\mu_{k}(s,\pi^+_{k}(s)) + \sum_{s'} \widetilde p_k(s'|s,\pi^+_{k}(s)) u_k^{(i)}(s') = \widetilde\mu_{k}\Big(c_{s,\pi^+_{k}(s)}\Big) + \sum_{s'} \widetilde p_{k}\Big(s'|c_{s,\pi^+_{k}(s)}\Big) u_k^{(i)}(s')\,,
}
%which can be written as:
%\begin{equation*}
%u_{i+1}(s) = \mu^+_{t_k}(c_{s,\pi^+_{t_k}(s)}) + \sum_{s'} p^+_{t_k}(s'|c_{s,\pi^+_{t_k}(s)})u_i(s')
%\end{equation*}
where for a given $(s,a)$, $c_{s,a} \in \cC$ denotes the cluster to which $(s,a)$ belongs. Substituting this into (\ref{eq:puterman_convergence}) gives
\begin{equation*}
\Big|\Big( g_k - \widetilde\mu_{k}\Big(c_{s,\pi^+_{k}(s)}\Big) \Big) - \Big(\sum_{s'} \widetilde p_{k}\Big(s'|c_{s,\pi^+_{k}(s)}\Big)u_k^{(i)}(s') - u_k^{(i)}(s)\Big)\Big|
\leq \frac{1}{\sqrt{t_k}}\, , \qquad \forall s\in \cS\, .
\end{equation*}
Defining
${\bf g}_k = g_k \mathbf 1$, $\widetilde{\boldsymbol{\mu}}_{k} := \big(\widetilde\mu_{k}\big(c_{s, \pi^+_{k}(s)}\big)\big)_s$, $\widetilde{\mathbf{P}}_k := \big(\widetilde p_{k}\big(s'|c_{s,\pi^+_{k}(s)}\big)\big)_{s, s'}$ and $\nu_{k} := \big(\nu_k\big(c_{s,\pi^+_{k}(s)}\big)\big)_s$, we can rewrite the above inequality as:
\begin{equation*}
\Big|{\bf g}_k - \widetilde{\boldsymbol{\mu}}_{k} - (\widetilde{\mathbf{P}}_k - \mathbf{I}) u_k^{(i)} \Big|
\leq \frac{1}{\sqrt{t_k}}\mathbf 1\,.
\end{equation*}
Combining this with (\ref{eq:delta_init}) yields
\begin{align}
\Delta_k&\leq \sum_{c \in \cC} \nu_k(c) \big(g_k-\mu(c)\big) + \sum_{c \in \cC} \frac{\nu_k(c)}{\sqrt{t_k}} \nonumber\\
&= \sum_{c \in \cC} \nu_k(c) \big( g_k - \widetilde\mu_{k}(c) \big) + \sum_{c \in \cC} \nu_k(c) \big( \widetilde\mu_{k}(c) - \mu(c) \big) + \sum_{c \in \cC}
\frac{\nu_k(c)}{\sqrt{t_k}} \nonumber\\
&\leq \nu_{k} (\widetilde{\mathbf{P}}_k - \mathbf{I} ) u_k^{(i)} + \sum_{c \in \cC} \nu_k(c) \big(\widetilde\mu_{k}(c) - \mu(c) \big) + 2 \sum_{c \in \cC} \frac{\nu_k(c)}{\sqrt{t_k}}\, .\nonumber
\end{align}
Similarly to \citep{jaksch2010near}, we define $w_k(s) := u_k^{(i)}(s) - \tfrac{1}{2}(\min_s u_k^{(i)}(s) + \max_s u_k^{(i)}(s))$ for all $s\in \cS$. Then, in view of the fact that $\widetilde{\mathbf{P}}_k$ is row-stochastic, we obtain



\begin{align}
\Delta_k&\leq \nu_{k} (\widetilde{\mathbf{P}}_k - \mathbf{I} ) w_k + \sum_{c \in \cC} \nu_k(c) \big(\widetilde \mu_{k}(c) - \mu(c) \big) + 2 \sum_{c \in \cC} \frac{\nu_k(c)}{\sqrt{t_k}}\, .
\end{align}
The second term in the right-hand side can be upper bounded as follows: $M \in \cM_{k}$ implies
\als{
\widetilde\mu_{k}(c) - \mu(c) &\leq |\widetilde\mu_{k}(c) - \widehat \mu_{k}(c)| + |\widehat \mu_{k}(c) - \mu(c)| \leq 2\beta'_{n_{k}(c)}(\tfrac{\delta}{2C}) \\
    &= 2\sqrt{\frac{1}{2n_{k}(c)}\Big(1\!+\!\frac{1}{n_{k}(c)}\Big)\log\Big(4C\sqrt{n_{k}(c)\!+\!1}/\delta\Big)} \\
    &\leq 2\sqrt{\frac{1}{n_k(c)}\log\big(4C\sqrt{T+1}/\delta\big)}\, ,
}
where we have used $1\leq n_k(c) \leq T$ in the last inequality. Using this bound and noting that $\max \{1,n_{k}(c)\} \leq t_k$, we obtain
\begin{align}
\Delta_k
&\leq \nu_{k} (\widetilde{\mathbf{P}}_k-\mathbf{I})w_k + 2\Big(\sqrt{\log\big(4C\sqrt{T+1}/\delta\big)} + 1\Big)
\sum_{c \in \cC} \frac{\nu_k(c)}{\sqrt{\max\{1, n_{k}(c)\}}}\, .
\label{eq:main_delta_minmk}
\end{align}
\end{comment}

In what follows, we derive an upper bound on $\nu_{k} (\widetilde{\mathbf{P}}_k-\mathbf{I})w_k$. Similarly to \citep{jaksch2010near}, we consider the following decomposition:
\als{
\nu_k(\widetilde{\mathbf{P}}_k - \mathbf{I}) w_k = \underbrace{\nu_k (\widetilde{\mathbf{P}}_k - \mathbf{P}_k) w_k}_{L_1(k)} + \underbrace{\nu_k (\mathbf{P}_k-\mathbf{I})w_k}_{L_2(k)} \, .
}
Noting that $\|w_k\|_\infty \leq \frac{D}{2}$, we upper bound $L_1(k)$ as follows:
\begin{align}
L_1(k) &\leq \sum_{s,a}\nu_k(s,a) \big(\widetilde p_{k}(s'|s,a) - p(s'|s,a)\big) w_k(s') \sk
&\leq \sum_{s,a} \nu_k(s,a) \|\widetilde p_{k}(\cdot|s,a)- p(\cdot|s,a) \|_1 \| w_k\|_\infty \sk
&\leq D \sum_{s,a} \nu_k(s,a) \bW_{n_{k}(c_{s,a})}(\tfrac{\delta}{C}) \sk
&= D \sum_{c\in \cC} \nu_k(c) \bW_{n_{k}(c)}(\tfrac{\delta}{C}) \sk
&\leq 2D \sqrt{\log\big(C2^{S}\sqrt{T+1}/\delta\big)} \sum_{c\in \cC} \frac{\nu_k(c)}{\sqrt{n_{k}(c)}} \, .
\label{eq:trans_prob_first_bound_minmk}
\end{align}


To upper bound $L_2(k)$, similarly to the
proof of \citep[Theorem~2]{jaksch2010near}, we define the  sequence $(X_t)_{t\geq 1}$, with $X_t := (p(\cdot|s_t,a_t) - \mathbf e_{s_{t+1}})w_{k_t}\bI\{M \in \cM_{k_t}\}$, for all $t$, where $k_t$ denotes the episode containing step $t$. Note that $\mathbb{E}[X_t|s_1, a_1, \dots, s_t, a_t] = 0$, so $(X_t)_{t\geq 1}$ is martingale difference sequence. Furthermore, $|X_t|\leq D$: Indeed, for all $t$, by the H\"{o}lder inequality,
$$
|X_t| \leq \|p(\cdot|s_t,a_t) - \mathbf e_{s_{t+1}}\|_1\|w_{k(t)}\|_\infty \leq \Big(\|p(\cdot|s_t,a_t)\|_1 + \|\mathbf e_{s_{t+1}}\|_1\Big)\frac{D}{2}  = D\,.
$$
Using similar steps as in \citep{jaksch2010near}, for any $k$ with $M \in \cM_{k}$, we have that:
\begin{align*}
L_2(k) &\leq \sum_{t=t_k}^{t_{k+1} -1} X_t + D\, ,
\end{align*}
so that $\sum_{k=1}^{m(T)} L_2(k) \leq \sum_{t=1}^T X_t +m(T)D$. Therefore, by  Lemma \ref{lem:time-uniform-AzumaHoeffding}, we deduce that with probability at least $1-\delta$,
\begin{align}
\sum_{k=1}^{m(T)} L_2(k) &\leq D \sqrt{2 (T+1) \log(\sqrt{T+1}/\delta)} + m(T)D \sk
&\leq D \sqrt{2 (T+1) \log(\sqrt{T+1}/\delta)}  + DC\log_2(\tfrac{8T}{C})\, ,
\label{eq:trans_prob_second_overall_minmk}
\end{align}
where the last step follows from Lemma \ref{lem:NbEpisodes}.

\paragraph{Final control.}Combing (\ref{eq:main_delta_minmk})--(\ref{eq:trans_prob_second_overall_minmk}) and summing over all episodes give:
\begin{align}
\sum_{k=1}^{m(T)} \Delta_k &\bI\{M \in \cM_{k}\} \leq
\sum_{k=1}^{m(T)} L_1(k) + \sum_{k=1}^{m(T)} L_2(k) + 2\Big(\sqrt{\log\big(C\sqrt{T+1}/\delta\big)} + 1\Big)\sum_{k=1}^{m(T)} \sum_{c \in \cC} \frac{\nu_k(c)}{\sqrt{n_{k}(c)}} \nonumber \\
&\leq 2\Big(D \sqrt{\log\big(C2^S\sqrt{T+1}/\delta\big)} + \sqrt{\log\big(C\sqrt{T+1}/\delta\big)} + 1\Big) \sum_{k=1}^{m(T)}
\sum_{c\in \cC} \frac{\nu_k(c)}{\sqrt{n_{k}(c)}}\nonumber\\
& + D\sqrt{ 2 (T+1) \log\big( \sqrt{T+1}/\delta\big)} + DC\log_2(\tfrac{8T}{C})	 \, ,	
\label{eq:trans_prob_intermed_minmk}
\end{align}
with probability at least $1-\delta$. To upper bound the right-hand side, we recall the following lemma:

\begin{lemma}[{\cite[Lemma~19]{jaksch2010near}}]\label{lem:sequence}
	For any sequence of numbers $z_1, z_2, \dots, z_n$ with $0 \leq z_k \leq Z_{k-1} := \max\{1, \sum_{i=1}^{k-1}z_i\}$,
	$$
	\sum_{k=1}^n 	\frac{z_k}{\sqrt{Z_{k-1}}} 	\leq 	\big(\sqrt{2} + 1\big) 	\sqrt{Z_n}\, .
	$$
\end{lemma}

Note that $n_{k}(c) = \sum_{k'<k} \nu_{k'}(c)$. Hence, applying Lemma \ref{lem:sequence} gives
\begin{equation*}
\sum_{c \in \cC} \sum_{k=1}^{m(T)} \frac{\nu_k(c)}{\sqrt{n_{k}(c)}}  \leq
\sum_{c \in \cC} \big(\sqrt{2} + 1\big) \sqrt{n_{m(T)}(c)} \le	\big( \sqrt{2} + 1 \big) \sqrt{CT}\, ,
\end{equation*}
where the last step follows from Jensen's inequality and $\sum_c n_{m(T)}(c) = T$. Therefore,
\begin{align*}
\sum_{k=1}^{m(T)} \Delta_k \bI\{M \in \cM_{k}\}
&\leq  D\sqrt{ 2 (T+1) \log\big( \sqrt{T+1}/\delta\big)} + DC\log_2(\tfrac{8T}{C}) \nonumber\\
&+ 2\big(\sqrt{2} + 1 \big)\Big(D \sqrt{\log\big(C2^{S}\sqrt{T+1}/\delta\big)} + \sqrt{\log\big(C\sqrt{T+1}/\delta\big)} + 1\Big)  \sqrt{CT}\, ,
\end{align*}
with probability of at least $1 - \delta$. Finally, the regret of \CUCRL($\cC,\sigma$) is controlled on an event of probability higher than $1-2\delta-\delta-\delta$, uniformly over all $T$,
by
\als{
\kR(T) &\leq 2\big(\sqrt{2} + 1\big)\Big(D \sqrt{\log\big(C2^{S}\sqrt{T+1}/\delta\big)} + \sqrt{\log\big(C\sqrt{T+1}/\delta\big)} + 1\Big)  \sqrt{CT}\\
& +D\sqrt{ 2 (T+1) \log\big( \sqrt{T+1}/\delta\big)} + DC\log_2(\tfrac{8T}{C}) + \sqrt{ \tfrac{1}{2}(T+1) \log\big( \sqrt{T+1}/\delta\big)}\\
&\leq 18\sqrt{CT\big(S + \log(C\sqrt{T+1}/\delta)\big)} +  DC\log_2(\tfrac{8T}{C}) \, ,}
thus completing the proof. We finally note that when the mean reward function is known, as in the main text, the above bound holds with a probability higher than $1-3\delta$.
\end{proof}


\subsection{Proof of Lemma \ref{lem:NbEpisodes}}
The proof uses similar steps as in the proof of Proposition 18 in \citep{jaksch2010near}.

Recall that given $c$, $N_T(c)$ and $\nu_k(c):=\nu_{t_k}(c)$ denote as the total number of state-action observations, up to step $T$ and in episode $k$, respectively. % there is a state-action class $c$ in each episode $k < m$ with $\nu_k(c) = n_{t_k}(c)$.
For any $c$, let $K(c)$ denote the number of episodes where a state-action pair from $c$ is sampled: $K(c)=\sum_{k=1}^{m(T)} \bI\{\nu_k(c)>0\}$. It is worth mentioning that if $n_{k}(c) > 0$ and $\nu_k(c) = n_{k}(c)$, by the design of the algorithm, $n_{k+1}(c) = 2n_{k}(c)$. Hence,
\als{
n_{m(T)}(c) = \sum_{k = 1}^{m(T)} \nu_k(c) \geq 	1 + \sum_{k: \nu_k(c) = n_{k}(c)}
n_{k}(c) 	\geq 	1 + \sum_{i = 1}^{K(c)}2^{i-1}  = 2^{K(c)} \, .
}

If $n_{m(T)}(c) = 0$, then $K(c) = 0$, so that $n_{m(T)}(c) \geq 2^{K(c)} - 1$ for all $c$. Thus,
\begin{equation*}
T = \sum_{c \in \cC} n_{m(T)}(c) \geq \sum_{c \in \cC} \big(2^{K(c)} - 1\big)
\end{equation*}
On the other hand, an episode has happened when either $n_{k}(c) = 0$ or $n_k(c) = \nu_k(c)$. Therefore, $m(T) \leq 1 + C + \sum_{c \in \cC} K(c)$ and consequently, $\sum_{c \in \cC} K(c) \geq m(T) - 1 - C$. Hence, by Jensen's inequality, we obtain
\begin{equation*}
\sum_{c \in \cC}2^{K(c)} \geq C2^{\sum_{c \in \cC}\frac{K(c)}{C}} \geq C2^{\frac{m(T)-1}{C}-1} \, .
\end{equation*}
Putting together, we obtain $T \geq C\big(2^{\frac{m(T)-1}{C} - 1} - 1\big)$. Therefore,
\begin{equation*}
m(T) \leq 1 + 2C + C\log_2(\tfrac{T}{C}) \leq 3C + C\log_2(\tfrac{T}{C}) \leq C\log_2(\tfrac{8T}{C})\, ,
\end{equation*}
thus concluding the proof.
\ep





==> New folder/definitions.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% COMMANDS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\ttt}{\texttt}

%%%%%%%%%%%%%% Proof
\newcommand{\bp}{\noindent{\emph{Proof}.}\ }
\newcommand{\ep}{\hfill $\Box$}

%%%%%%%%%%%%%% Equations
\newcommand{\BEAS}{\begin{eqnarray*}}
\newcommand{\EEAS}{\end{eqnarray*}}
\newcommand{\BEA}{\begin{eqnarray}}
\newcommand{\EEA}{\end{eqnarray}}
\newcommand{\BEQ}{\begin{equation}}
\newcommand{\EEQ}{\end{equation}}
\newcommand{\BIT}{\begin{itemize}}
\newcommand{\EIT}{\end{itemize}}
\newcommand{\BNUM}{\begin{enumerate}}
\newcommand{\ENUM}{\end{enumerate}}
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\beqa}{\begin{eqnarray}}
\newcommand{\eeqa}{\end{eqnarray}}
\newcommand{\beqan}{\begin{eqnarray*}}
\newcommand{\eeqan}{\end{eqnarray*}}
\newcommand{\bealn}{\begin{align*}}
\newcommand{\eealn}{\end{align*}}
\newcommand{\al}[1]{ \begin{align} #1  \end{align}}
\newcommand{\eq}[1]{ \begin{equation} #1  \end{equation}}
\newcommand{\als}[1]{ \begin{align*} #1  \end{align*}}
\newcommand{\eqs}[1]{ \begin{equation*} #1  \end{equation*}}
\newcommand{\sk}{\nonumber\\}
%\newcommand{\eqdef}{\stackrel{\textrm{def}}{=}}
%\newcommand{\eqdefemph}{\stackrel{\textrm{\emph{def}}}{=}}
\def\NoNumber#1{{\def\alglinenumber##1{}\State #1}\addtocounter{ALG@line}{-1}}

%%%%%%%%%%%%%% Misc
\newcommand{\Lp}{\left(}
\newcommand{\Rp}{\right)}
\newcommand{\Lb}{\left[}
\newcommand{\Rb}{\right]}
\newcommand{\vs}{\vspace{0.2in}}
\newcommand{\hs}{\hspace{0.5in}}
\newcommand{\el}{\end{flushleft}}
\newcommand{\bl}{\begin{flushleft}}
\newcommand{\floor}[1]{  \lfloor #1 \rfloor}
\newcommand{\ceil}[1]{  \lceil #1 \rceil}
\newcommand{\inff}{\operatornamewithlimits{inf}}
\newcommand{\tto}[1]{\underset{#1}{\to}}
\newcommand{\eqdist}{\,{\buildrel d \over =}\,}
\renewcommand{\baselinestretch}{.98}
\newcommand{\iskip}{{\vskip -0.4cm}}
\newcommand{\siskip}{{\vskip -0.2cm}}
\newcommand{\fix}{\marginpar{FIX}}
\newcommand{\new}{\marginpar{NEW}}
\newcommand{\argmin}{\arg\!\min}
\newcommand{\argmax}{\arg\!\max}
\newcommand{\Argmax}{\mathop{\mathrm{Argmax}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% MATH SYMBOLS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\bA}{\mathbb{A}}
\newcommand{\bB}{\mathbb{B}}
\newcommand{\bC}{\mathbb{C}}
\newcommand{\bD}{\mathbb{D}}
\newcommand{\bE}{\mathbb{E}}
\newcommand{\bF}{\mathbb{F}}
\newcommand{\bG}{\mathbb{G}}
\newcommand{\bH}{\mathbb{H}}
\newcommand{\bI}{\mathbb{I}}
\newcommand{\bJ}{\mathbb{J}}
\newcommand{\bK}{\mathbb{K}}
\newcommand{\bL}{\mathbb{L}}
\newcommand{\bM}{\mathbb{M}}
\newcommand{\bN}{\mathbb{N}}
\newcommand{\bO}{\mathbb{O}}
\newcommand{\bP}{\mathbb{P}}
\newcommand{\bQ}{\mathbb{Q}}
\newcommand{\bR}{\mathbb{R}}
\newcommand{\bS}{\mathbb{S}}
\newcommand{\bT}{\mathbb{T}}
\newcommand{\bU}{\mathbb{U}}
\newcommand{\bV}{\mathbb{V}}
\newcommand{\bW}{\mathbb{W}}
\newcommand{\bX}{\mathbb{X}}
\newcommand{\bY}{\mathbb{Y}}
\newcommand{\bZ}{\mathbb{Z}}

\newcommand{\cA}{\mathcal{A}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cJ}{\mathcal{J}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cZ}{\mathcal{Z}}

\newcommand{\kA}{\mathfrak{A}}
\newcommand{\kB}{\mathfrak{B}}
\newcommand{\kC}{\mathfrak{C}}
\newcommand{\kD}{\mathfrak{D}}
\newcommand{\kE}{\mathfrak{E}}
\newcommand{\kF}{\mathfrak{F}}
\newcommand{\kG}{\mathfrak{G}}
\newcommand{\kH}{\mathfrak{H}}
\newcommand{\kI}{\mathfrak{I}}
\newcommand{\kJ}{\mathfrak{J}}
\newcommand{\kK}{\mathfrak{K}}
\newcommand{\kL}{\mathfrak{L}}
\newcommand{\kM}{\mathfrak{M}}
\newcommand{\kN}{\mathfrak{N}}
\newcommand{\kO}{\mathfrak{O}}
\newcommand{\kP}{\mathfrak{P}}
\newcommand{\kQ}{\mathfrak{Q}}
\newcommand{\kR}{\mathfrak{R}}
\newcommand{\kS}{\mathfrak{S}}
\newcommand{\kT}{\mathfrak{T}}
\newcommand{\kU}{\mathfrak{U}}
\newcommand{\kV}{\mathfrak{V}}
\newcommand{\kW}{\mathfrak{W}}
\newcommand{\kX}{\mathfrak{X}}
\newcommand{\kY}{\mathfrak{Y}}
\newcommand{\kZ}{\mathfrak{Z}}

\newcommand{\bsym}{\boldsymbol}
\newcommand{\Real}{\mathbb{R}}
\newcommand{\Nat}{\mathbb{N}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\ind}{\mathbb{I}}
\newcommand{\indic}{\mathbb{I}}
\newcommand{\indOne}{\mathbbmss{1} }
\renewcommand{\phi}{\varphi}
\renewcommand{\epsilon}{\varepsilon}
%\renewcommand{\leq}{\leqslant}
%\renewcommand{\geq}{\geqslant}
%\renewcommand{\hat}{\widehat}

\def\M{{\mathbb M}}
\def\N{{\mathbb N}}
\def\NN{{\mathbb N}}
\def\EE{{\mathbb E}}
\def\PP{{\mathbb P}}
\def\RR{{\mathbb R}}
\def\ore{\overrightarrow{e}}
\def\orE{\overrightarrow{E}}
\def\ole{\overleftarrow{e}}
\def\d{\partial}
\def\bx{\bold{x}}
\def\bw{\bold{w}}
\def\bB{\bold{B}}
\def\Poi{\text{Poi}}
\def\Bin{\text{Bin}}
\def\odeg{\overline{\text{deg}}}
\def\Acal{{\mathcal A}}
\def\Pcal{{\mathcal P}}
\def\Rcal{{\mathcal R}}
\def\Dcal{{\mathcal D}}
\def\Ccal{{\mathcal C}}
\def\Ical{{\mathcal I}}
\def\Ocal{{\mathcal O}}
\def\Qcal{{\mathcal Q}}
\def\Bcal{{\mathcal B}}
\def\Hcal{{\mathcal H}}
\def\Ecal{{\mathcal E}}
\def\Fcal{{\mathcal F}}
\def\Ncal{{\mathcal N}}
\def\Mcal{{\mathcal M}}
\def\Lcal{{\mathcal L}}
\def\Kcal{{\mathcal K}}
\def\Gcal{{\mathcal G}}
\def\Scal{{\mathcal S}}
\def\Tcal{{\mathcal T}}
\def\Ucal{{\mathcal U}}
\def\Vcal{{\mathcal V}}
\def\Xcal{{\mathcal X}}
\def\Zcal{{\mathcal Z}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% ABBREVIATIONS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\Span}{\bS}
\newcommand{\Esp}{\mathbb{E}}
\newcommand{\Var}{\mathbb{V}}
\newcommand{\var}{\mathbb{V}}
\renewcommand{\Pr}{\mathbb{P}}
\newcommand{\Normal}{\cN}
\newcommand{\Bern}{\mathrm{Ber}}
\newcommand{\bias}{b}
\newcommand{\Spanstar}{\Psi}
\newcommand{\supp}{\mathrm{supp}}
\newcommand{\llnp}{\mathrm{llnp}}
\newcommand{\kl}{\texttt{KL}}
\newcommand{\KL}{\texttt{KL}}
\newcommand{\klber}{\texttt{kl}}
\newcommand{\klg}{\texttt{KLG}}
\newcommand{\regret}{\mathfrak{R}}
\newcommand{\SP}{\textrm{SP}}

\newcommand{\ucb}{\textsc{\texttt{UCB1}}}
\newcommand{\klucb}{\textsc{\texttt{KL-UCB}}}
\newcommand{\TS}{\textsc{\texttt{TS}}}
\newcommand{\Ucrl}{\textsc{\texttt{Ucrl2}}}
\newcommand{\UCRL}{\textsc{\texttt{Ucrl2}}}
\newcommand{\UCRLLaplace}{\textsc{\texttt{Ucrl2-L}}}
\newcommand{\KLUCRL}{\textsc{\texttt{KL-Ucrl}}}
%\newcommand{\BK}{\textsc{\texttt{Burnetas-Katehakis}}}
\newcommand{\BK}{\texttt{BK}}
\newcommand{\OLP}{\textsc{\texttt{OLP}}}
\newcommand{\regal}{\textsc{\texttt{Regal}}}
\newcommand{\QL}{\textsc{\texttt{Q-Learning}}}
\newcommand{\EVI}{\textsc{\texttt{Extended Value Iteration}}}
\newcommand{\geo}{\mathrm{geo}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% MISC %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\setlength{\belowdisplayskip}{0pt}
\setlength{\abovedisplayskip}{0pt}
\setlength{\belowdisplayshortskip}{0pt}
\setlength{\abovedisplayshortskip}{0pt}



==> definitions.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% COMMANDS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\ttt}{\texttt}

%%%%%%%%%%%%%% Proof
\newcommand{\bp}{\noindent{\emph{Proof}.}\ }
\newcommand{\ep}{\hfill $\Box$}

%%%%%%%%%%%%%% Equations
\newcommand{\BEAS}{\begin{eqnarray*}}
\newcommand{\EEAS}{\end{eqnarray*}}
\newcommand{\BEA}{\begin{eqnarray}}
\newcommand{\EEA}{\end{eqnarray}}
\newcommand{\BEQ}{\begin{equation}}
\newcommand{\EEQ}{\end{equation}}
\newcommand{\BIT}{\begin{itemize}}
\newcommand{\EIT}{\end{itemize}}
\newcommand{\BNUM}{\begin{enumerate}}
\newcommand{\ENUM}{\end{enumerate}}
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\beqa}{\begin{eqnarray}}
\newcommand{\eeqa}{\end{eqnarray}}
\newcommand{\beqan}{\begin{eqnarray*}}
\newcommand{\eeqan}{\end{eqnarray*}}
\newcommand{\bealn}{\begin{align*}}
\newcommand{\eealn}{\end{align*}}
\newcommand{\al}[1]{ \begin{align} #1  \end{align}}
\newcommand{\eq}[1]{ \begin{equation} #1  \end{equation}}
\newcommand{\als}[1]{ \begin{align*} #1  \end{align*}}
\newcommand{\eqs}[1]{ \begin{equation*} #1  \end{equation*}}
\newcommand{\sk}{\nonumber\\}
%\newcommand{\eqdef}{\stackrel{\textrm{def}}{=}}
%\newcommand{\eqdefemph}{\stackrel{\textrm{\emph{def}}}{=}}
\def\NoNumber#1{{\def\alglinenumber##1{}\State #1}\addtocounter{ALG@line}{-1}}

%%%%%%%%%%%%%% Misc
\newcommand{\Lp}{\left(}
\newcommand{\Rp}{\right)}
\newcommand{\Lb}{\left[}
\newcommand{\Rb}{\right]}
\newcommand{\vs}{\vspace{0.2in}}
\newcommand{\hs}{\hspace{0.5in}}
\newcommand{\el}{\end{flushleft}}
\newcommand{\bl}{\begin{flushleft}}
\newcommand{\floor}[1]{  \lfloor #1 \rfloor}
\newcommand{\ceil}[1]{  \lceil #1 \rceil}
\newcommand{\inff}{\operatornamewithlimits{inf}}
\newcommand{\tto}[1]{\underset{#1}{\to}}
\newcommand{\eqdist}{\,{\buildrel d \over =}\,}
\renewcommand{\baselinestretch}{.98}
\newcommand{\iskip}{{\vskip -0.4cm}}
\newcommand{\siskip}{{\vskip -0.2cm}}
\newcommand{\fix}{\marginpar{FIX}}
\newcommand{\new}{\marginpar{NEW}}
\newcommand{\argmin}{\arg\!\min}
\newcommand{\argmax}{\arg\!\max}
\newcommand{\Argmax}{\mathop{\mathrm{Argmax}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% MATH SYMBOLS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\bA}{\mathbb{A}}
\newcommand{\bB}{\mathbb{B}}
\newcommand{\bC}{\mathbb{C}}
\newcommand{\bD}{\mathbb{D}}
\newcommand{\bE}{\mathbb{E}}
\newcommand{\bF}{\mathbb{F}}
\newcommand{\bG}{\mathbb{G}}
\newcommand{\bH}{\mathbb{H}}
\newcommand{\bI}{\mathbb{I}}
\newcommand{\bJ}{\mathbb{J}}
\newcommand{\bK}{\mathbb{K}}
\newcommand{\bL}{\mathbb{L}}
\newcommand{\bM}{\mathbb{M}}
\newcommand{\bN}{\mathbb{N}}
\newcommand{\bO}{\mathbb{O}}
\newcommand{\bP}{\mathbb{P}}
\newcommand{\bQ}{\mathbb{Q}}
\newcommand{\bR}{\mathbb{R}}
\newcommand{\bS}{\mathbb{S}}
\newcommand{\bT}{\mathbb{T}}
\newcommand{\bU}{\mathbb{U}}
\newcommand{\bV}{\mathbb{V}}
\newcommand{\bW}{\mathbb{W}}
\newcommand{\bX}{\mathbb{X}}
\newcommand{\bY}{\mathbb{Y}}
\newcommand{\bZ}{\mathbb{Z}}

\newcommand{\cA}{\mathcal{A}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cJ}{\mathcal{J}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cZ}{\mathcal{Z}}

\newcommand{\kA}{\mathfrak{A}}
\newcommand{\kB}{\mathfrak{B}}
\newcommand{\kC}{\mathfrak{C}}
\newcommand{\kD}{\mathfrak{D}}
\newcommand{\kE}{\mathfrak{E}}
\newcommand{\kF}{\mathfrak{F}}
\newcommand{\kG}{\mathfrak{G}}
\newcommand{\kH}{\mathfrak{H}}
\newcommand{\kI}{\mathfrak{I}}
\newcommand{\kJ}{\mathfrak{J}}
\newcommand{\kK}{\mathfrak{K}}
\newcommand{\kL}{\mathfrak{L}}
\newcommand{\kM}{\mathfrak{M}}
\newcommand{\kN}{\mathfrak{N}}
\newcommand{\kO}{\mathfrak{O}}
\newcommand{\kP}{\mathfrak{P}}
\newcommand{\kQ}{\mathfrak{Q}}
\newcommand{\kR}{\mathfrak{R}}
\newcommand{\kS}{\mathfrak{S}}
\newcommand{\kT}{\mathfrak{T}}
\newcommand{\kU}{\mathfrak{U}}
\newcommand{\kV}{\mathfrak{V}}
\newcommand{\kW}{\mathfrak{W}}
\newcommand{\kX}{\mathfrak{X}}
\newcommand{\kY}{\mathfrak{Y}}
\newcommand{\kZ}{\mathfrak{Z}}

\newcommand{\bsym}{\boldsymbol}
\newcommand{\Real}{\mathbb{R}}
\newcommand{\Nat}{\mathbb{N}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\ind}{\mathbb{I}}
\newcommand{\indic}{\mathbb{I}}
\newcommand{\indOne}{\mathbbmss{1} }
\renewcommand{\phi}{\varphi}
\renewcommand{\epsilon}{\varepsilon}
%\renewcommand{\leq}{\leqslant}
%\renewcommand{\geq}{\geqslant}
%\renewcommand{\hat}{\widehat}

\def\M{{\mathbb M}}
\def\N{{\mathbb N}}
\def\NN{{\mathbb N}}
\def\EE{{\mathbb E}}
\def\PP{{\mathbb P}}
\def\RR{{\mathbb R}}
\def\ore{\overrightarrow{e}}
\def\orE{\overrightarrow{E}}
\def\ole{\overleftarrow{e}}
\def\d{\partial}
\def\bx{\bold{x}}
\def\bw{\bold{w}}
\def\bB{\bold{B}}
\def\Poi{\text{Poi}}
\def\Bin{\text{Bin}}
\def\odeg{\overline{\text{deg}}}
\def\Acal{{\mathcal A}}
\def\Pcal{{\mathcal P}}
\def\Rcal{{\mathcal R}}
\def\Dcal{{\mathcal D}}
\def\Ccal{{\mathcal C}}
\def\Ical{{\mathcal I}}
\def\Ocal{{\mathcal O}}
\def\Qcal{{\mathcal Q}}
\def\Bcal{{\mathcal B}}
\def\Hcal{{\mathcal H}}
\def\Ecal{{\mathcal E}}
\def\Fcal{{\mathcal F}}
\def\Ncal{{\mathcal N}}
\def\Mcal{{\mathcal M}}
\def\Lcal{{\mathcal L}}
\def\Kcal{{\mathcal K}}
\def\Gcal{{\mathcal G}}
\def\Scal{{\mathcal S}}
\def\Tcal{{\mathcal T}}
\def\Ucal{{\mathcal U}}
\def\Vcal{{\mathcal V}}
\def\Xcal{{\mathcal X}}
\def\Zcal{{\mathcal Z}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% ABBREVIATIONS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\Span}{\bS}
\newcommand{\Esp}{\mathbb{E}}
\newcommand{\Var}{\mathbb{V}}
\newcommand{\var}{\mathbb{V}}
\renewcommand{\Pr}{\mathbb{P}}
\newcommand{\Normal}{\cN}
\newcommand{\Bern}{\mathrm{Ber}}
\newcommand{\bias}{b}
\newcommand{\Spanstar}{\Psi}
\newcommand{\supp}{\mathrm{supp}}
\newcommand{\llnp}{\mathrm{llnp}}
\newcommand{\kl}{\texttt{KL}}
\newcommand{\KL}{\texttt{KL}}
\newcommand{\klber}{\texttt{kl}}
\newcommand{\klg}{\texttt{KLG}}
\newcommand{\regret}{\mathfrak{R}}
\newcommand{\SP}{\textrm{SP}}

\newcommand{\ucb}{\textsc{\texttt{UCB1}}}
\newcommand{\klucb}{\textsc{\texttt{KL-UCB}}}
\newcommand{\TS}{\textsc{\texttt{TS}}}
\newcommand{\Ucrl}{\textsc{\texttt{Ucrl2}}}
\newcommand{\UCRL}{\textsc{\texttt{Ucrl2}}}
\newcommand{\UCRLLaplace}{\textsc{\texttt{Ucrl2-L}}}
\newcommand{\KLUCRL}{\textsc{\texttt{KL-Ucrl}}}
%\newcommand{\BK}{\textsc{\texttt{Burnetas-Katehakis}}}
\newcommand{\BK}{\texttt{BK}}
\newcommand{\OLP}{\textsc{\texttt{OLP}}}
\newcommand{\regal}{\textsc{\texttt{Regal}}}
\newcommand{\QL}{\textsc{\texttt{Q-Learning}}}
\newcommand{\EVI}{\textsc{\texttt{Extended Value Iteration}}}
\newcommand{\geo}{\mathrm{geo}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% MISC %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\setlength{\belowdisplayskip}{0pt}
\setlength{\abovedisplayskip}{0pt}
\setlength{\belowdisplayshortskip}{0pt}
\setlength{\abovedisplayshortskip}{0pt}


